Asking Multimodal Clarifying Questions in Mixed-Initiative Conversational Search

In mixed-initiative conversational search systems, clarifying questions are used to help users who struggle to express their intentions in a single query. These questions aim to uncover user's information needs and resolve query ambiguities. We hypothesize that in scenarios where multimodal information is pertinent, the clarification process can be improved by using non-textual information. Therefore, we propose to add images to clarifying questions and formulate the novel task of asking multimodal clarifying questions in open-domain, mixed-initiative conversational search systems. To facilitate research into this task, we collect a dataset named Melon that contains over 4k multimodal clarifying questions, enriched with over 14k images. We also propose a multimodal query clarification model named Marto and adopt a prompt-based, generative fine-tuning strategy to perform the training of different stages with different prompts. Several analyses are conducted to understand the importance of multimodal contents during the query clarification phase. Experimental results indicate that the addition of images leads to significant improvements of up to 90% in retrieval performance when selecting the relevant images. Extensive analyses are also performed to show the superiority of Marto compared with discriminative baselines in terms of effectiveness and efficiency.

==> sections/XX-human-evaluation.tex <==
% \moh{Mohammad stopped here.}
\section{Human Evaluation}
% I feel like this section won't fit here since we are referring to the model which we are yet to discuss
\subsection{Annotation}
To understand the importance of images in the task of query clarification, we carry out a human evaluation with assessors from \ac{AMT} platform. We sample positive and negative questions from \OurData, 100 each to run the evaluation on. These questions are selected based on the question classification model which predicts whether a question would benefit more from image attachment or not. The assessors have access to the user information need (facets), the query, and the clarifying question with three images. We ask the assessors to judge the questions and images on four aspects namely: \textit{suitability, relevance, understandable} and \textit{useful} by answering the following questions.


\begin{itemize}[leftmargin=*]
    \item Is the question suitable for image attachment?
    \item Which of the images are relevant to the question?
    \item Which of the images make the question understandable?
    \item Which of the images are useful to the question?
\end{itemize}

\noindent
\textit{Suitability} refers to whether humans agree with the model predictions on whether the question would benefit from image attachment. 
For \textit{relevance}, the images associated with a question are judged if they are on the same topic aspect as the question. The \textit{understandable} aspect assesses whether the attached images allow the user to have a clear picture of what the system is referring to. Whereas the \textit{useful} aspect captures the ability of the images to convey visual messages in relation to the questions.

Each question was assessed by five workers and in total the evaluation was conducted on 200 questions. We use simple majority, that is, the final label is determined unless three or more assessors agreed on it. 

\subsection{Analysis}
In Table~\ref{tab:no.questions} and \ref{tab:no.images} we show the percentage of questions and images where three or more assessors agreed on a label. Out of the 200 questions used in this experiment, 96\% were judged as suitable for image association regardless of 50\% of the questions being selected from the negative class. This indicates that though the images hurt the model performance it is not the same case when it comes to user experience. Users tend to prefer engaging with multimodal content compared to single modality. From the open comments provided by assessors on the significance of the images, we note that most assessors agree on the useful information images add to a textual clarification question. In addition the images are important when a user is in exploration mode and not looking for something specific as they provide possibilities of what is available.

For relevance ~93\% of the questions had at least one image on the same topic as the question and more than 50\% of the images were judged as relevant. Despite this we still realize that close to half of the images were found by assessors not to be on the same topic as the question. Associating irrelevant images may lead to an ineffective model and hurt user experience during interaction. Therefore it is important to ensure the attached images are on the same topic as the question, which motivates the image selection module in \OurModel to retrieve the top 1 relevant image. 
%\cs{This statement is down playing our annotation, not sure how to place it.}

More images were judged as relevant compared to useful~(42.5\%) and understandable~(36.5\%) with an average of one image per question for both aspects. Our analysis indicate that when only one image was selected as relevant then 95\% of the times the image was also useful. This is because the images were not only on the same topic as the question but had other useful visual information too such as comparison tables. Where two or more images were selected as relevant on average one of the image was selected as useful. In cases where more than one image was selected as relevant and useful, from examining the images we found out that the images represented different aspects of the questions. For example a question regarding `teddy bear' with images representing the size, types and colors of available teddy bears, will have the three images selected as both relevant and useful.
%\cs{This motivates our image selection module to ensure to get the top 1 relevant image as each question on average had one relevant image.}
% Tables~\ref{tab:no.questions}  represent the statistics of the annotated questions and images. Though the experiment was conducted with 50\% positive cases and another 50\% negative cases predicted by the question selection model, the assessors judge 93\% of the questions as suitable for image association. 51\% of the images were selected as relevant with an average of one relevant images per question. 32.5\% of the images made the question more understandable and 42.5\% of the images conveyed visual messages.

In general, though not all questions may benefit from image attachment during retrieval, we have shown that the image content is useful to users during query clarification phase. Most assessors note the addition of context and making the questions more understandable as the most significant contributions of the images. In addition we also note that during answer collection phase in our annotation, compared to ClariQ, \OurData answers were long and detailed which improves the model's accuracy during document retrieval.

\begin{table}[!t]\small
    \centering
     \caption{Number of questions suitable for image attachment, with relevant, understandable and useful images.}
    \begin{tabular}{l c}
    \toprule
        Aspect & \% of questions \\
        \midrule
        Suitability & 96 \\ 
        Relevant & 93.5 \\
        Understandable & 84 \\
        Useful & 89 \\
        \bottomrule
    \end{tabular}
    \label{tab:no.questions}
\end{table}

\begin{table}[!t]\small
    \centering
    \caption{Statistics of images that were judged as relevant, understandable and useful}
    \begin{tabular}{l c c}
    \toprule
        Aspect & \% of images & Avg. images \\
        \midrule
        Relevant & 50.1 & 1\\
        Understandable & 36.5 & 1\\
        Useful & 42.5& 1 \\
        \bottomrule
    \end{tabular}
    
    \label{tab:no.images}
\end{table}

% \header{Suitability}   \\
% \header{Relevant}51\% of the images were judges as being relevant to the question. On average two image were selected as relevant per question.\\
% \header{Useful} \\
% \header{Understandable}


==> sections/introduction-original.tex <==
\section{Introduction}
Traditional search systems often struggle to provide relevant results meeting a user's information need when they encounter incomplete or ambiguous queries.
To effectively tackle this problem, considerable research efforts have been carried out towards query clarification~\cite{Zamani2020GeneratingCQ,AliannejadiSigir19,Aliannejadi2021AnalysingMI}, which aims to enable a system to determine whether it should   ask questions proactively to clarify users’ information need before presenting a result list. Specifically, each time when the user and a conversational system interact, the system decides whether a clarifying question is necessary~\cite{Hancock2019LearningFD}. The system then selects/generates the most suitable clarifying question~\cite{Rao2018LearningTA},  which results in an enhanced user experience, creating a more natural interaction and 
ultimately achieving superior retrieval outcomes.
% By clarifying unclear or incomplete queries, this system can 
% enhancing user experience while creating a more natural interaction, with potentially better retrieval outcomes for the user.

\textbf{Motivation.} 
Although query clarification serves as a valuable tool in conversational systems, several drawbacks remain that can limit its effectiveness in retrieving relevant information. 
% Importantly, real-life conversations tend to involve knowledge from more than one modality, such as images, text, and speech~\cite{Liao2021MMConvAE}. 
First of all, operating based on a single mode of communication (i.e., text), the system may not be able to understand the intent of the user accurately, especially in cases where the query is ambiguous or incomplete~\cite{Sundar2022MultimodalCA}. Moreover, since real-life conversations tend to involve knowledge from more than one modality, the reliance on a single mode of communication limits the communication between users and systems, hindering the unimodal clarification system to provide a more  natural interaction that mirrors human-to-human conversations~\cite{Liao2021MMConvAE}.
Finally, the lack of visual appeal in unimodal search systems could result in decreased engagement and user satisfaction, which could have a negative impact on the user experience~\cite{Muftah2020InvestigatingTE,Berget2016IsVC}. 
% Overall, the exclusive reliance on a single mode of communication can hinder the ability of monomodal clarification systems to provide accurate and effective results for users. can lead to decreased user satisfaction with the search experience

Motivated by these insights, there are recent proposals that aim to expand the clarification process to include multimodal information for  providing a better search experience~\citep{Sundar2022MultimodalCA}. 
Fig.~\ref{fig:exmaple} illustrates the idea.
%
\begin{figure}[!h]
    \centering
    \vspace*{-1mm}
    \includegraphics[width=0.65\linewidth]{sections/Figures/Figure1.pdf}
    \caption{An example of incorporating multimodal information into the query  clarification phase.}
    \label{fig:exmaple}
    \vspace*{-1mm}
\end{figure}
%
When a user inputs a query ``teddy bear'' with the underlying information need of ``help me find a teddy bear to buy as a present'', compared with  plain text questions, outputting a clarifying question with images of different sizes of teddy bears helps the user more directly realize what they are searching for. 
Via such multimodal interactions, useful but implicit knowledge is conveyed through images, potentially leading to improved retrieval performance and a better grasp of the user's intention.


\textbf{The MQC task.} 
In this study, we formulate the task of asking multimodal clarifying questions in open-domain mixed-initiative conversational search systems. 
Specifically, we define \ac{MQC} as \textit{asking clarifying questions that involve both text and images in a text-dominant conversation}. 
To provide context for this task, we present the workflow depicted in Figure~\ref{fig:workflow}.
Initially, the user submits a search query to a conversational search system. 
The system retrieves relevant documents and assesses their suitability for presentation to the user. In cases where the query is ambiguous or the system fails to understand the user's intent, a clarifying question is selected or generated. 
In contrast to text-only query clarification, our approach employs a classifier to determine whether to include images in the clarifying question. 
Upon confirmation (this type of question defined as \textbf{multimodal clarifying question}), multiple images are retrieved and displayed to the user alongside the clarifying question. The provision of visual information enhances the user's comprehension, permitting a more informed response.  The user's response, together with the multimodal clarifying question, are then processed to improve document retrieval and provide precise and pertinent retrieval results.

\textbf{Data collection and analysis.} 
To anchor our work in data and facilitate the offline evaluation of the MQC system, we collect a new dataset, \emph{\OurData} (\textbf{M}ultimodal qu\textbf{e}ry c\textbf{l}arification conversati\textbf{on}s), based on an existing text-only clarifying question dataset. \OurData contains over 4k multimodal clarifying questions with over 14k images. 70\% of the clarifying questions originate from the ClariQ dataset~\citep{Aliannejadi2020ConvAI3GC}; the remaining 30\% are collected from scratch. To ensure the reliability of \OurData, we undertake various quality control measures. Subsequently, we perform several analyses to gain a better understanding of the significance of multimodal content in the query clarification process and its impact on users.  Our analysis of  \OurData shows that the usage of images during the clarification phase leads to more contextualized answers, resulting in richer semantic information compared to the text-only ClariQ dataset. 

\textbf{Representation learning for multimodal clarification.} 
We propose \emph{\OurModel} (\textbf{M}ultimod\textbf{a}l que\textbf{r}y clarifica\textbf{t}ion m\textbf{o}del), a model for representation learning of multimodal clarifying questions. 
\OurModel is based on a pre-trained multimodal generative model that takes images and text as input. 
We adopt a multi-task fine-tuning approach to train different stages of \OurModel with different prompts under a unified  structure. In detail, \OurModel is initially trained to generate true or false labels for a given clarifying question to assess if a question is suitable to be accompanied by images. For true cases, an image is selected based on similarity to the question.
Inspired by generative retrieval techniques in text-only retrieval~\cite{Lee2022ContextualizedGR,DeCao2020AutoregressiveER}, we design a multimodal generative document retrieval method where all questions with or without images are trained to generate document IDs. By leveraging pre-trained knowledge, this approach equips \OurData with enhanced retrieval ability in an end-to-end manner.

To assess the performance of \OurModel, we compare it  with several competitive unimodal and multimodal document retrieval baselines. Our findings demonstrate that multimodal clarifying questions have a positive impact on the retrieval task compared to unimodal baselines. Additionally, we find that generative models outperform discriminative models in terms of effectiveness and efficiency. These insights can aid the development of more advanced conversational search systems that take advantage of the rich information conveyed by multimodal interactions.
% Thus, \OurModel unifies different subtasks of multimodal query clarification into a single framework. 

\yifei{Might need to move the research questions to somewhere else}

\textbf{Research questions.}
We answer the following research questions:
\begin{enumerate*}[label=(\textbf{RQ\arabic*}),nosep]
    \item How can we incorporate images into the query clarification pipeline and  evaluate it in an offline setting? 
    \item Does asking multimodal clarifying questions influence user response?
    \item Are generative document retrieval models more effective and efficient for multimodal clarification? 
    \item What is the effect of images on the document retrieval task and how sensitive is it to the addition of images?
\end{enumerate*} 

% \textbf{Main findings.}
 

% We conduct further analyses on \OurModel to investigate the role of images in multimodal clarifying questions under various scenarios. 

\textbf{Contributions.} 
In summary, our contributions are as follows:
\begin{itemize}[leftmargin=*,nosep]
    \item We define the task of \ac{MQC} in a mixed-initiative conversational search system, which adds image information in clarifying questions to improve the downstream document retrieval task. 
    \item We propose a benchmark dataset, called \OurData, to perform offline evaluation of the system. It contains over 4k multimodal clarifying questions, enriched with over 14k images.\footnote{Link to the data and code repository will be added upon paper's acceptance.}
    \item We propose \OurModel, a model that adopts a prompt-based generative fine-tuning pipeline for representation learning of multimodal clarifying questions. We show that it outperforms competitive baselines for the document retrieval downstream task.
\end{itemize}


==> sections/notes.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{ccccc}
%          & Suitability & Relevant &Understandable & Useful \\
%          \midrule
%           & 931~(93\%) & & &  \\
%         Image 1 & &445~(44.5\%) &566~(56.6\%) &335~(33.5\%)  \\
%         Image 2 & &602~(60.2\%) &397~(39.7\%) &566~(56.6\%)  \\
%         Image 3 & &456~(45.6\%) &317~(31.7\%) & 472~(47.2\%) \\
%         None & &44~(0.04\%) & 130~(0.13\%)& 54~(0.05\%) \\
%     \end{tabular}
%     \caption{}
%     \label{tab:my_label}
% \end{table}


\begin{table}[]
    \centering
    \begin{tabular}{cccc}
         & Relevant &Understandable & Useful \\
         \midrule
        
        Image 1 &75 &123 &44 \\
        image 2 &127 &64 &119\\
        image 3 & 118& 32 & 92\\
        None & 0&2 & 0 \\
        No-agreement & 13 & 30 & 22
        
    \end{tabular}
    \caption{Table showing out 200 questions used for human evaluation, how many times were the images selected as relevant, understandable or useful}
    \label{tab:my_label}
\end{table}

image1: relevant: 21 : understanding: 85, useful: 13
image2: relevant: 55, understanding: 30, useful: 60
image3: relevant: 26, understanding: 9, useful: 36
no agreement: relevant: 13, understanding: 30, useful: 22        
no agreement for all aspects: 6 - Find out what happened?
all images: relevant: 15, understanding: 8, useful: 10 - What is common when all images are selected for all aspects?
all images all aspects: 3
image1 in total: relevant:75, understanding
image2: relevant: , understanding: 64

Criteria, if an image is selected by three or more annotators- simple majority
Out of 600 images only :\\
98\% of questions required image attachment\\
320 images out of 600 were relevant ~50\% of the images\\
219 images out 600 made the annotator understand the question better ~36.5\% \\
255 images out of 600 were found to have useful visual messages ~42.5\% \\
relevant: two images: 75 out of 200, one image:102, all images: \\
understanding: two images:36, one image: 124, \\
useful: 57, one image: 109\\
Cooccurence rel-useful: one image = 97, two images: 41\\
only one image for all aspects:12\\
all images for all aspects: 4\\
When an image was selected as relevant some percentage times it was likely to be useful too 97 out of 102

